Magnetic Component of Quark-Gluon Plasma is also a Liquid!

The so called magnetic scenario recently suggested in \cite{Liao_ES_mono} emphasizes the role of monopoles in strongly coupled quark-gluon plasma (sQGP) near/above the deconfinement temperature, and specifically predicts that they help reduce its viscosity by the so called "magnetic bottle" effect. Arguments for "magnetic liquid" in 1-2$T_c$ based on lattice measurement of monopole density were provided in \cite{Chernodub}. Here we present results for monopole-(anti)monopole correlation functions from the same classical molecular dynamics simulations, which are found to be in very good agreement with recent lattice results \cite{D'Alessandro:2007su}. We show that the magnetic Coulomb coupling does run in the direction $opposite$ to the electric one, as expected, and it is roughly inverse of the asymptotic freedom formula for the electric one. However, as $T$ decreases to $T_c$, the magnetic coupling never gets weak, with the plasma parameter always large enough ($\Gamma>1$). This nicely agrees with empirical evidences from RHIC experiments, implying that magnetic objects cannot have large mean free path and should also form a good liquid with low viscosity.

==> wideabs <==
  You can actually get a first page that looks something like the first
page of Phys. Rev. (with abstract across the page), IF you are using
version 3.1 of REVTeX. Here is the general format:

\wideabs{
\title{ . . . }
   .
   .
   .
\pacs{ . . . }
}

That is, just insert the command \wideabs the title, and put the
ending curly brace after the pacs.

  Note that these lines should never appear in a file destined for the APS.
Note also that this is a quick hack and may have unknown drawbacks, along
with these known ones:

  (1) Byline footnotes (any footnotes or \thanks between the inserted lines)
      will probably just disappear.
  (2) No catcode changes can be effected between the inserted lines;
      mainly this means no verbatim and \verb, but may have other
      consequences.
It was intended to produce a style that had the abstract printed on the
width of the page, but there were always problems with the implementation and
so it was withdrawn near the release date. It may be possible to solve this
problem in the future.





